Temporal Interpolation as an Unsupervised Pretraining Task for Optical Flow Estimation

The difficulty of annotating training data is a major obstacle to using CNNs for low-level tasks in video. Synthetic data often does not generalize to real videos, while unsupervised methods require heuristic losses. Proxy tasks can overcome these issues, and start by training a network for a task for which annotation is easier or which can be trained unsupervised. The trained network is then fine-tuned for the original task using small amounts of ground truth data. Here, we investigate frame interpolation as a proxy task for optical flow. Using real movies, we train a CNN unsupervised for temporal interpolation. Such a network implicitly estimates motion, but cannot handle untextured regions. By fine-tuning on small amounts of ground truth flow, the network can learn to fill in homogeneous regions and compute full optical flow fields. Using this unsupervised pre-training, our network outperforms similar architectures that were trained supervised using synthetic optical flow.

==> sections/00_abstract.tex <==
\begin{abstract}
The difficulty of annotating training data is a major obstacle to using convolutional neural networks (CNNs) for low-level tasks in video.
Synthetic data is usually used to overcome this problem, but such data often does not generalize well to real videos.
Fully unsupervised methods, on the other hand, usually require heuristics as part of the loss function.
A way to address these issues is to use proxy tasks, which starts by training a network for a task for which annotated data is easier to come across, or which can be trained in an unsupervised fashion.
The resulting network can then be fine-tuned for the original task using small amounts of annotated ground truth data.
In this work, we investigate the use of frame interpolation as a proxy task for optical flow estimation.
To this end, we train a CNN unsupervised to perform temporal interpolation using approximately one million samples gathered from real movies.
While such a network already implicitly estimates some correspondences, the critical component of fill-in of uniform regions is missing, since it is not required to solve the interpolation task.
We show how fine-tuning on optical flow can learn such fill-in and compute full optical flow fields, and that good accuracy can already be achieved using only a small amount of annotated ground truth.

On both synthetic and real data, our network outperforms similar architectures that were trained purely with synthetic data, demonstrating the importance of learning correspondences from real data.
Furthermore, while not explicitly designed for good temporal interpolation performance, our network nevertheless achieves better results than state-of-the-art, specialized architectures.

\end{abstract}

